prDeep: Robust Phase Retrieval with a Flexible Deep Network

Phase retrieval algorithms have become an important component in many modern computational imaging systems. For instance, in the context of ptychography and speckle correlation imaging, they enable imaging past the diffraction limit and through scattering media, respectively. Unfortunately, traditional phase retrieval algorithms struggle in the presence of noise. Progress has been made recently on more robust algorithms using signal priors, but at the expense of limiting the range of supported measurement models (e.g., to Gaussian or coded diffraction patterns). In this work we leverage the regularization-by-denoising framework and a convolutional neural network denoiser to create prDeep, a new phase retrieval algorithm that is both robust and broadly applicable. We test and validate prDeep in simulation to demonstrate that it is robust to noise and can handle a variety of system models. A MatConvNet implementation of prDeep is available at https://github.com/ricedsp/prDeep.

==> PhaseRetreivalAlgs.tex <==
\section{Phase Retrieval}

GS
HIO
...
Cite Tom's paper to show that few algorithms are significantly better than HIO.

D-prGAMP
prVAMP
RED-DnCNN

Ashok said writing up RED phase retrieval here is worth doing.

==> Ptychography.tex <==
\section{Ptychography}
Need algorithms that work with overlapping Fourier measurements. In most contexts, accuracy is of primary concern.

==> TM.tex <==
\section{Coherent Inverse Scattering}
Need fast algorithms that work with $\{0,1\}$ measurements.

==> training.tex <==
\section{Training and Initialization}
